Chemo-Dynamical Tagging in the Outskirts: The Origins of Stellar Substructures in the Magellanic Clouds

We present the first detailed chemical analysis from APOGEE-2S observations of stars in six regions of recently discovered substructures in the outskirts of the Magellanic Clouds extending to 20 degrees from the LMC center. We also present, for the first time, the metallicity and alpha-abundance radial gradients of the LMC and SMC out to 11 degrees and 6 degrees, respectively. Our chemical tagging includes 13 species including light, alpha, and Fe-peak elements. We find that the abundances of all of these chemical elements in stars populating two regions in the northern periphery - along the northern "stream"-like feature - show good agreement with the chemical patterns of the LMC, and thus likely have an LMC origin. For substructures located in the southern periphery of the LMC, we find more complex chemical and kinematical signatures, indicative of a mix of LMC-like and SMC-like populations. However, the southern region closest to the LMC shows better agreement with the LMC, whereas that closest to the SMC shows a much better agreement with the SMC chemical pattern. When combining this information with 3-D kinematical information for these stars, we conclude that the southern region closest to the LMC has likely an LMC origin, whereas that closest to the SMC has an SMC origin, and the other two southern regions have a mix of LMC and SMC origins. Our results add to the evidence that the southern substructures of the LMC periphery are the product of close interactions between the LMC and SMC, and thus likely hold important clues that can constrain models of their detailed dynamical histories.

==> authors.tex <==
\author[0000-0002-8129-3487]{C\'esar Mu\~noz}
\institute{Instituto Multidisciplinario de Investigaci\'on y Postgrado, Universidad de La Serena, Ra\'ul Bitr\'an 1305, La Serena, Chile}
\institute{Departamento de Astronom\'ia, Universidad de La Serena, Av. Cisternas 1200, La Serena, Chile}

\author[0000-0003-2325-9616]{Antonela Monachesi}
\institute{Instituto Multidisciplinario de Investigaci\'on y Postgrado, Universidad de La Serena, Ra\'ul Bitr\'an 1305, La Serena, Chile}
\institute{Departamento de Astronom\'ia, Universidad de La Serena, Av. Cisternas 1200, La Serena, Chile}

\author[0000-0002-1793-3689]{David L. Nidever}
\institute{Department of Physics, Montana State University, P.O. Box 173840, Bozeman, MT 59717, USA}

\author[0000-0003-2025-3147]{Steven R. Majewski}
\institute{Department of Astronomy, University of Virginia, Charlottesville, VA 22904-4325, USA}

\author[0000-0002-7009-3957]{Xinlun Cheng}
\institute{Department of Astronomy, University of Virginia, Charlottesville, VA 22904-4325, USA}

\author[0000-0002-7134-8296]{Knut Olsen}
\institute{National Optical-Infrared Astronomy Research Laboratory (NOIRLab), 950 North Cherry Avenue, Tucson, AZ 85719, USA}

\author[0000-0003-1680-1884]{Yumi Choi}
\institute{Department of Astronomy, University of California, Berkeley, 501 Campbell Hall 3411, CA 94720-3411, USA}

\author{Paul Zivick}
\institute{IQVIA}

\author{Douglas Geisler}
\institute{Instituto Multidisciplinario de Investigaci\'on y Postgrado, Universidad de La Serena, Ra\'ul Bitr\'an 1305, La Serena, Chile}
\institute{Departamento de Astronom\'ia, Universidad de La Serena, Av. Cisternas 1200, La Serena, Chile}
\institute{Departamento de Astronom\'ia, Casilla 160-C, Universidad de Concepci\'on, Concepci\'on, Chile.}


\author{Andres Almeida}
\institute{Department of Astronomy, University of Virginia, Charlottesville, VA 22904-4325, USA}

\author{Ricardo R. Mu\~noz}
\institute{Departamento de Astronom{\'i}a, Universidad de Chile, Camino El Observatorio 1515, Las Condes, Chile}

\author{Christian  Nitschelm}
\institute{ Centro de Astronom{\'i}a (CITEVA), Universidad de Antofagasta, Avenida Angamos 601, Antofagasta 1270300, Chile}

\author{Alexandre Roman-Lopes}
\institute{Departamento de Astronom\'ia, Universidad de La Serena, Av. Cisternas 1200, La Serena, Chile}

\author{Richard R. Lane}
\institute{Instituto de Astrof´ısica, Pontificia Universidad Cat´olica de Chile, Av. Vicuna Mackenna 4860, 782-0436 Macul, Santiago, Chile}

